Fifteen years of millimeter accuracy lunar laser ranging with APOLLO: dataset characterization

We present data from the Apache Point Observatory Lunar Laser-ranging Operation (APOLLO) covering the 15-year span from April 2006 through the end of 2020. APOLLO measures the earth-moon separation by recording the round-trip travel time of photons from the Apache Point Observatory to five retro-reflector arrays on the moon. The APOLLO data set, combined with the 50-year archive of measurements from other lunar laser ranging (LLR) stations, can be used to probe fundamental physics such as gravity and Lorentz symmetry, as well as properties of the moon itself. We show that range measurements performed by APOLLO since 2006 have a median nightly accuracy of 1.7 mm, which is significantly better than other LLR stations.

==> Makefile <==
# specify the color type (x=col or x=bw)

x ?= col
v ?= 1

all:
	pdflatex "\def\FIGCOLORTYPE{_$(x)}\input{np}"
	bibtex np
	pdflatex "\def\FIGCOLORTYPE{_$(x)}\input{np}"
	pdflatex "\def\FIGCOLORTYPE{_$(x)}\input{np}"

diff:
	git latexdiff --output np_diff.pdf --no-view --main np.tex HEAD~$(v) --

arxiv:
	tar -czvf np.tar.gz Makefile np.tex np.bbl Journal_Abbrevs.tex iopart.cls iopart12.clo img/np_per_year_all_stations.pdf img/observing_session_durations.pdf img/np_per_session.pdf img/days_between_sessions.pdf img/observing_session_times.pdf img/np_per_reflector_vs_time.pdf img/refl_per_session.pdf img/nights_per_reflector.pdf img/np_uncertainty_distribution.pdf img/nightly_uncertainty.pdf img/lunar_phase_by_np.pdf

clean:
	rm -f *~ *.log *.bbl *.aux *.blg


